A Block-Based Testing Framework for Scratch

Block-based programming environments like Scratch are widely used in introductory programming courses. They facilitate learning pivotal programming concepts by eliminating syntactical errors, but logical errors that break the desired program behaviour are nevertheless possible. Finding such errors requires testing, i.e., running the program and checking its behaviour. In many programming environments, this step can be automated by providing executable tests as code; in Scratch, testing can only be done manually by invoking events through user input and observing the rendered stage. While this is arguably sufficient for learners, the lack of automated testing may be inhibitive for teachers wishing to provide feedback on their students' solutions. In order to address this issue, we introduce a new category of blocks in Scratch that enables the creation of automated tests. With these blocks, students and teachers alike can create tests and receive feedback directly within the Scratch environment using familiar block-based programming logic. To facilitate the creation and to enable batch processing sets of student solutions, we extend the Scratch user interface with an accompanying test interface. We evaluated this testing framework with 28 teachers who created tests for a popular Scratch game and subsequently used these tests to assess and provide feedback on student implementations. An overall accuracy of 0.93 of teachers' tests compared to manually evaluating the functionality of 21 student solutions demonstrates that teachers are able to create and effectively use tests. A subsequent survey confirms that teachers consider the block-based test approach useful.

==> assets/big_table.tex <==
\begin{tabular}{lrrrrrrrrrrrl}
\toprule
 & #Tests & # Students Evaluated & Test vs Golden & Test vs Feedback & Feedback vs Golden & Changes better & # Changes & Pass To Fail Correct & Fail To Pass Correct & Pass To Fail Wrong & Fail To Pass Wrong & Name \\
\midrule
0 & 6 & 5 & 0.682540 & 0.766667 & 0.900000 & 0.714286 & 7 & 5.000000 & 0.000000 & 2.000000 & 0.000000 & Andreas Freundl \\
1 & 6 & 21 & 0.944444 & 0.928571 & 0.888889 & 0.111111 & 9 & 0.000000 & 1.000000 & 6.000000 & 2.000000 & Andreas Michl \\
2 & 6 & 21 & 0.833333 & 1.000000 & 0.833333 & NaN & 0 & NaN & NaN & NaN & NaN & Artem Frelich \\
3 & 6 & 7 & 0.944444 & 0.904762 & 0.833333 & 0.000000 & 4 & 0.000000 & 0.000000 & 2.000000 & 2.000000 & Bianca Kuhnert \\
4 & 6 & 21 & 0.936508 & 0.896825 & 0.960317 & 0.615385 & 13 & 6.000000 & 2.000000 & 4.000000 & 1.000000 & Dennis Ohlwerter \\
5 & 6 & 21 & 0.952381 & 0.968254 & 0.920635 & 0.000000 & 4 & 0.000000 & 0.000000 & 1.000000 & 3.000000 & Edi \\
6 & 6 & 21 & 0.960317 & 0.960317 & 0.968254 & 0.600000 & 5 & 1.000000 & 2.000000 & 2.000000 & 0.000000 & Felix Platzer \\
7 & 5 & 10 & 0.801587 & 0.833333 & 0.933333 & 0.800000 & 10 & 0.000000 & 8.000000 & 0.000000 & 2.000000 & Ines Jobst \\
8 & 6 & 21 & 0.992063 & 0.984127 & 0.976190 & 0.000000 & 2 & 0.000000 & 0.000000 & 2.000000 & 0.000000 & Johannes Ebner \\
9 & 6 & 5 & 0.880952 & 0.966667 & 0.933333 & 1.000000 & 1 & 0.000000 & 1.000000 & 0.000000 & 0.000000 & Karin Lanner \\
10 & 6 & 21 & 0.809524 & 0.984127 & 0.793651 & 0.000000 & 2 & 0.000000 & 0.000000 & 1.000000 & 1.000000 & Lisa Bailey \\
11 & 6 & 5 & 0.785714 & 0.966667 & 0.800000 & 0.000000 & 1 & 0.000000 & 0.000000 & 1.000000 & 0.000000 & Magdalena Miethaner \\
12 & 4 & 21 & 0.642857 & 0.833333 & 0.563492 & 0.142857 & 14 & 2.000000 & 0.000000 & 5.000000 & 7.000000 & Martin Schuderer \\
13 & 6 & 21 & 0.952381 & 0.976190 & 0.976190 & 1.000000 & 3 & 0.000000 & 3.000000 & 0.000000 & 0.000000 & Maximilian Richter \\
14 & 6 & 21 & 0.936508 & 0.992063 & 0.928571 & 0.000000 & 1 & 0.000000 & 0.000000 & 1.000000 & 0.000000 & Michael Berglehner \\
15 & 6 & 8 & 0.873016 & 0.937500 & 0.833333 & 0.333333 & 3 & 1.000000 & 0.000000 & 2.000000 & 0.000000 & Michael Ramich \\
16 & 2 & 4 & 0.198413 & 0.272727 & 0.166667 & 0.250000 & 8 & 0.000000 & 2.000000 & 2.000000 & 4.000000 & Nicole Plass \\
17 & 6 & 21 & 0.817460 & 0.968254 & 0.817460 & 0.500000 & 4 & 2.000000 & 0.000000 & 0.000000 & 2.000000 & Roland Goerge \\
18 & 6 & 21 & 0.944444 & 0.984127 & 0.928571 & 0.000000 & 2 & 0.000000 & 0.000000 & 2.000000 & 0.000000 & Silvia Gehring \\
19 & 6 & 21 & 0.936508 & 0.904762 & 0.952381 & 0.583333 & 12 & 2.000000 & 5.000000 & 3.000000 & 2.000000 & Simon Ludwig \\
20 & 6 & 12 & 0.992063 & 1.000000 & 1.000000 & NaN & 0 & NaN & NaN & NaN & NaN & Stefan Mayr \\
21 & 6 & 21 & 0.952381 & 0.904762 & 0.952381 & 0.500000 & 12 & 4.000000 & 2.000000 & 3.000000 & 3.000000 & Stefan Nömer \\
22 & 4 & 5 & 0.611111 & 0.678571 & 0.900000 & 0.888889 & 9 & 0.000000 & 8.000000 & 0.000000 & 1.000000 & Tanja Sabine Nuber \\
23 & 4 & 5 & 0.642857 & 1.000000 & 0.666667 & NaN & 0 & NaN & NaN & NaN & NaN & Thomas Umlauf \\
24 & 6 & 21 & 1.000000 & 0.968254 & 0.968254 & 0.000000 & 4 & 0.000000 & 0.000000 & 3.000000 & 1.000000 & Tobias Fuchs \\
25 & 6 & 21 & 0.944444 & 0.936508 & 0.976190 & 0.750000 & 8 & 0.000000 & 6.000000 & 2.000000 & 0.000000 & Tobias Hausinger \\
26 & 5 & 5 & 0.571429 & 0.586207 & 0.866667 & 0.833333 & 12 & 0.000000 & 10.000000 & 1.000000 & 1.000000 & Verena Riederer \\
27 & 6 & 21 & 0.920635 & 1.000000 & 0.920635 & NaN & 0 & NaN & NaN & NaN & NaN & Zsuzsanna Huber \\
\bottomrule
\end{tabular}


==> assets/evaluated_vs_muster.tex <==
\begin{tabular}{lrrrrr}
\toprule
 & Fitting & Not Fitting & Answered Functionalities & # Students Evaluated & Evaluated per Student \\
\midrule
0 & 0.900000 & 0.100000 & 0.238095 & 5 & 6.000000 \\
1 & 0.888889 & 0.111111 & 1.000000 & 21 & 6.000000 \\
2 & 0.833333 & 0.166667 & 1.000000 & 21 & 6.000000 \\
3 & 0.833333 & 0.166667 & 0.333333 & 7 & 6.000000 \\
4 & 0.960317 & 0.039683 & 1.000000 & 21 & 6.000000 \\
5 & 0.920635 & 0.079365 & 1.000000 & 21 & 6.000000 \\
6 & 0.968254 & 0.031746 & 1.000000 & 21 & 6.000000 \\
7 & 0.933333 & 0.066667 & 0.476190 & 10 & 6.000000 \\
8 & 0.976190 & 0.023810 & 1.000000 & 21 & 6.000000 \\
9 & 0.933333 & 0.066667 & 0.238095 & 5 & 6.000000 \\
10 & 0.793651 & 0.206349 & 1.000000 & 21 & 6.000000 \\
11 & 0.800000 & 0.200000 & 0.238095 & 5 & 6.000000 \\
12 & 0.563492 & 0.436508 & 1.000000 & 21 & 6.000000 \\
13 & 0.976190 & 0.023810 & 1.000000 & 21 & 6.000000 \\
14 & 0.928571 & 0.071429 & 1.000000 & 21 & 6.000000 \\
15 & 0.833333 & 0.166667 & 0.380952 & 8 & 6.000000 \\
16 & 0.166667 & 0.833333 & 0.190476 & 4 & 6.000000 \\
17 & 0.817460 & 0.182540 & 1.000000 & 21 & 6.000000 \\
18 & 0.928571 & 0.071429 & 1.000000 & 21 & 6.000000 \\
19 & 0.952381 & 0.047619 & 1.000000 & 21 & 6.000000 \\
20 & 1.000000 & 0.000000 & 0.571429 & 12 & 6.000000 \\
21 & 0.952381 & 0.047619 & 1.000000 & 21 & 6.000000 \\
22 & 0.900000 & 0.100000 & 0.238095 & 5 & 6.000000 \\
23 & 0.666667 & 0.333333 & 0.238095 & 5 & 6.000000 \\
24 & 0.968254 & 0.031746 & 1.000000 & 21 & 6.000000 \\
25 & 0.976190 & 0.023810 & 1.000000 & 21 & 6.000000 \\
26 & 0.866667 & 0.133333 & 0.238095 & 5 & 6.000000 \\
27 & 0.920635 & 0.079365 & 1.000000 & 21 & 6.000000 \\
\bottomrule
\end{tabular}


==> assets/evaluated_vs_sample_per_functionality.tex <==
\begin{tabular}{lrrrrrr}
\toprule
 & Init & Move & Crash text & Crash costume & Win text & Win costume \\
\midrule
Same & 0.941589 & 0.876168 & 0.873832 & 0.939252 & 0.775701 & 0.943925 \\
Different & 0.058411 & 0.123832 & 0.126168 & 0.060748 & 0.224299 & 0.056075 \\
Amount & 428.000000 & 428.000000 & 428.000000 & 428.000000 & 428.000000 & 428.000000 \\
\bottomrule
\end{tabular}


==> assets/evaluated_vs_test.tex <==
\begin{tabular}{lrrr}
\toprule
 & Same as Test & Not Same as Test & Tests written \\
\midrule
0 & 0.766667 & 0.233333 & 6 \\
1 & 0.928571 & 0.071429 & 6 \\
2 & 1.000000 & 0.000000 & 6 \\
3 & 0.904762 & 0.095238 & 6 \\
4 & 0.896825 & 0.103175 & 6 \\
5 & 0.968254 & 0.031746 & 6 \\
6 & 0.960317 & 0.039683 & 6 \\
7 & 0.833333 & 0.166667 & 5 \\
8 & 0.984127 & 0.015873 & 6 \\
9 & 0.966667 & 0.033333 & 6 \\
10 & 0.984127 & 0.015873 & 6 \\
11 & 0.966667 & 0.033333 & 6 \\
12 & 0.833333 & 0.166667 & 4 \\
13 & 0.976190 & 0.023810 & 6 \\
14 & 0.992063 & 0.007937 & 6 \\
15 & 0.937500 & 0.062500 & 6 \\
16 & 0.272727 & 0.727273 & 2 \\
17 & 0.968254 & 0.031746 & 6 \\
18 & 0.984127 & 0.015873 & 6 \\
19 & 0.904762 & 0.095238 & 6 \\
20 & 1.000000 & 0.000000 & 6 \\
21 & 0.904762 & 0.095238 & 6 \\
22 & 0.678571 & 0.321429 & 4 \\
23 & 1.000000 & 0.000000 & 4 \\
24 & 0.968254 & 0.031746 & 6 \\
25 & 0.936508 & 0.063492 & 6 \\
26 & 0.586207 & 0.413793 & 5 \\
27 & 1.000000 & 0.000000 & 6 \\
\bottomrule
\end{tabular}


==> assets/test_vs_evaluated_per_functionality.tex <==
\begin{tabular}{lrrrrrr}
\toprule
 & Init & Move & Crash text & Crash costume & Win text & Win costume \\
\midrule
Same & 0.955504 & 0.927570 & 0.945946 & 0.955189 & 0.898990 & 0.954545 \\
Different & 0.044496 & 0.072430 & 0.054054 & 0.044811 & 0.101010 & 0.045455 \\
Amount & 427.000000 & 428.000000 & 407.000000 & 424.000000 & 396.000000 & 418.000000 \\
\bottomrule
\end{tabular}


==> assets/test_vs_sample.tex <==
\begin{tabular}{lrrr}
\toprule
 & Same as Sample & Not Same as Sample & Tests written \\
\midrule
0 & 0.682540 & 0.317460 & 6 \\
1 & 0.944444 & 0.055556 & 6 \\
2 & 0.833333 & 0.166667 & 6 \\
3 & 0.944444 & 0.055556 & 6 \\
4 & 0.936508 & 0.063492 & 6 \\
5 & 0.952381 & 0.047619 & 6 \\
6 & 0.960317 & 0.039683 & 6 \\
7 & 0.801587 & 0.198413 & 5 \\
8 & 0.992063 & 0.007937 & 6 \\
9 & 0.880952 & 0.119048 & 6 \\
10 & 0.809524 & 0.190476 & 6 \\
11 & 0.785714 & 0.214286 & 6 \\
12 & 0.642857 & 0.357143 & 4 \\
13 & 0.952381 & 0.047619 & 6 \\
14 & 0.936508 & 0.063492 & 6 \\
15 & 0.873016 & 0.126984 & 6 \\
16 & 0.198413 & 0.801587 & 2 \\
17 & 0.817460 & 0.182540 & 6 \\
18 & 0.944444 & 0.055556 & 6 \\
19 & 0.936508 & 0.063492 & 6 \\
20 & 0.992063 & 0.007937 & 6 \\
21 & 0.952381 & 0.047619 & 6 \\
22 & 0.611111 & 0.388889 & 4 \\
23 & 0.642857 & 0.357143 & 4 \\
24 & 1.000000 & 0.000000 & 6 \\
25 & 0.944444 & 0.055556 & 6 \\
26 & 0.571429 & 0.428571 & 5 \\
27 & 0.920635 & 0.079365 & 6 \\
\bottomrule
\end{tabular}


==> assets/test_vs_sample_per_functionality.tex <==
\begin{tabular}{lrrrrrr}
\toprule
 & Init & Move & Crash text & Crash costume & Win text & Win costume \\
\midrule
Same & 0.904762 & 0.841837 & 0.835034 & 0.947279 & 0.630952 & 0.867347 \\
Different & 0.095238 & 0.158163 & 0.164966 & 0.052721 & 0.369048 & 0.132653 \\
Amount & 588.000000 & 588.000000 & 588.000000 & 588.000000 & 588.000000 & 588.000000 \\
\bottomrule
\end{tabular}

